Compressive Coded Aperture Keyed Exposure Imaging with Optical Flow Reconstruction

This paper describes a coded aperture and keyed exposure approach to compressive video measurement which admits a small physical platform, high photon efficiency, high temporal resolution, and fast reconstruction algorithms. The proposed projections satisfy the Restricted Isometry Property (RIP), and hence compressed sensing theory provides theoretical guarantees on the video reconstruction quality. Moreover, the projections can be easily implemented using existing optical elements such as spatial light modulators (SLMs). We extend these coded mask designs to novel dual-scale masks (DSMs) which enable the recovery of a coarse-resolution estimate of the scene with negligible computational cost. We develop fast numerical algorithms which utilize both temporal correlations and optical flow in the video sequence as well as the innovative structure of the projections. Our numerical experiments demonstrate the efficacy of the proposed approach on short-wave infrared data.

==> CCA_macros.tex <==
\RequirePackage{color}
\usepackage{mathrsfs}
\usepackage{amsmath,amssymb,latexsym,subfigure}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage[pdftex]{graphicx}

% Example definitions.
% --------------------

\renewcommand{\vec}[1]{\boldsymbol{#1}}
\newcommand{\mat}[1]{\boldsymbol{\uppercase{#1}}}
\newcommand{\oper}[1]{\boldsymbol{\mathcal{#1}}}
\newcommand{\wh}[1]{{\widehat{#1}}}
\newcommand{\wt}[1]{{\widetilde{#1}}}
\def\expect{{\rm I\!\!E}}
\def\x{{\mathbf x}}
\def\L{{\cal L}}
\def\Re{\mathbb{R}}
\def\ones{\mathbb{1}}
\newcommand{\ints}{{\mathbb{Z}}}
\def \Poisson{{{\rm Poisson}}}
\def\deq{\triangleq}
\def\hf{\wh{f}}
\def\tf{f^{\star}}
\def\ttheta{\theta^{\star}}
\def\tif{\wt{f}}
\def\ttheta{\theta^{\star}}
\def\htheta{\wh{\theta}}
\def\argmin{\mathop{\arg \min}}
\def\pen{\mathop{\rm pen}}
\def\sP{\mathcal P}
\def\th{^{\rm th}}
\def\bI{\mathbb{I}}
\def\argmin{\mathop{\!\arg \min}}
\def\minimize{\mathop{\textrm{minimize}}}
\def\st{\mathop{\textrm{\!subject to}}}
\def\grad{\nabla}
\def\tv{{\rm TV}}
\newenvironment{squishlist}
{   \begin{list}{$\bullet$}
    { \setlength{\itemsep}{2pt}      \setlength{\parsep}{2pt}
      \setlength{\topsep}{0pt}       \setlength{\partopsep}{0pt}
      \setlength{\leftmargin}{1.5em} \setlength{\labelwidth}{1em}
      \setlength{\labelsep}{0.5em} } }
      {\end{list}}

\def\Re{I\!\!R}
\def\bfNt{\mathbf{n}_t}
\def\bfY{\mathbf{y}}
\def\bfYt{\mathbf{y}_t}
\def\bfYto{\mathbf{y}_{t+1}}
\def\bfRt{\mathbf{R}_t}
\def\bfAt{\mathbf{A}_t}
\def\bfA{\mathbf{A}}
\def\bfB{\mathbf{B}}
\def\bfC{\mathbf{C}}
\def\bfR{\mathbf{R}}
\def\bfW{\mathbf{W}}
\def\bfF{\mathbf{F}}
\def\bfN{\mathbf{n}}
\def\bfXt{\mathbf{x}_t}
\def\bfFt{\mathbf{f}_t}
\def\bfF{\mathbf{f}}
\def\bfthetat{\mathbf{\theta}_t}
\def\bftheta{\mathbf{\theta}}
\def\bfAtW{\mathbf{A}_{t,\mathbf{W}}}
\def\bfD{\mathbf{D}}
\def\bfh{\mathbf{h}}
\def\bfcapH{\mathbf{H}}
\def\bfC{\mathbf{C}}
\def\Deltait{\mathit{\Delta}}
\def\vect{{\textrm {vect}}}
\def\vtheta{\vec{\theta}}
\def\hmura{\mat{H}^{\rm MURA}}
\def\hcca{\mat{H}^{\rm CCA}}
\def\htcca{\tilde{\mat{H}}^{\rm CCA}}
\def\htcca{\mat{\tilde{H}}^{\rm CCA}}
\def\hrecon{\mat{H}^{\rm recon}}
\def\pcca{\mat{P}^{\rm CCA}}
\def\pmura{\mat{P}^{\rm MURA}}
\def\thcca{\mat{H}^{0}}
\def\Acca{\mat{A}^{\rm CCA}}
\def\TV{\oper{TV}}
\def\tA{\mat{A}^{0}}
\def\ty{\vec{y}^{0}}
\def\hcd{h^{\rm (CD)}}
\def\htmura{\wt{h}^{\rm (MURA)}}
\def\deq{\triangleq}
\def\argmin{\mathop{\arg \min}}
\def\fstar{\vec{f}^{\star}}
\def\gstar{\vec{g}^{\star}}
\def\Fstar{\mat{F}^{\star}}
\def\fest{\vec{\wh{f}}}
\def\Fest{\mat{\wh{F}}}
%\def\gstar{\vec{g}^{\rm true}}
\def\tstar{\vec{\theta}^{\star}}
\def\Gstar{\mat{G}^{\star}}
\def\Gest{\wh{\mat{G}}}
\def\gest{\wh{\vec{g}}}
\def\test{\vec{\wh{\theta}}}
\def\vtheta{\vec{\theta}}
\def\sP{\mathcal P}
\def\P{\mat{P}}
\def\downsamp{\oper{D}}
\def\sub{\mathop{{\text{subject to}}}}
\def\g{\vec{g}}
\def\f{\vec{f}}
\def\F{\mat{F}}
\def\G{\mat{G}}
\def\vW{\vec{w}}

\def\FF{\mathcal{F}}
\def\FFD{\mat{\mathcal{F}}_{2D}}
\def\IF{\FF^{-1}}
\def\IFD{\mat{\mathcal{F}}_{2D}^{-1}}
 \def \ie{{\em i.e., }}

\newtheorem{thm}{Theorem}

\newenvironment{myproof}
{\noindent{\sc Proof:}}
{$\square$ \\}

\newcommand{\todo}[1]{{\textcolor{red}{[#1]}}}
\newenvironment{todo2}
{\color{red}}{\color{black}}
\usepackage{booktabs}

\newcommand{\eref}[1]{(\ref{#1})}

